Play time with determinants

In this brief semi-expository article we present a few efficient techniques for calculating and proving determinantal identities. Several stimulating examples of different flavor and applications are spread across the pages which we hope the reader will find of particular interest.

==> 0137059.tex <==
%auto-ignore
